PUSHing Core-Collapse Supernovae to Explosions in Spherical Symmetry III: Nucleosynthesis Yields

In a previously presented proof-of-principle study, we established a parametrized spherically symmetric explosion method (PUSH) that can reproduce many features of core-collapse supernovae for a wide range of pre-explosion models. The method is based on the neutrino-driven mechanism and follows collapse, bounce and explosion. There are two crucial aspects of our model for nucleosynthesis predictions. First, the mass cut and explosion energy emerge simultaneously from the simulation (determining, for each stellar model, the amount of Fe-group ejecta). Second, the interactions between neutrinos and matter are included consistently (setting the electron fraction of the innermost ejecta). In the present paper, we use the successful explosion models from Ebinger et al. (2018) which include two sets of pre-explosion models at solar metallicity, with combined masses between 10.8 and 120 M$_{\odot}$. We perform systematic nucleosynthesis studies and predict detailed isotopic yields. The resulting $^{56}$Ni ejecta are in overall agreement with observationally derived values from normal core-collapse supernovae. The Fe-group yields are also in agreement with derived abundances for metal-poor star HD84937. We also present a comparison of our results with observational trends in alpha element to iron ratios.

==> niti_table.tex <==
\begin{center}
\begin{longtable*}{|c|llll|}

\multicolumn{5}{c}%
{{\bfseries \tablename\ \thetable{} -- Isotopic yields in M~$_{\odot}$ for all models}} \label{tab:nitis02}\\

\hline
\multicolumn{1}{|c|}{\textbf{Model}} & \multicolumn{1}{c}{\textbf{$^{56}$Ni}} & \multicolumn{1}{c}{\textbf{$^{57}$Ni}} & \multicolumn{1}{c}{\textbf{$^{58}$Ni}} & \multicolumn{1}{c|}{\textbf{$^{44}$Ti}}\\ 
\endfirsthead

\multicolumn{5}{c}%
{{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\
\hline
\multicolumn{1}{|c|}{\textbf{Model}} & \multicolumn{1}{c}{\textbf{$^{56}$Ni}} & \multicolumn{1}{c}{\textbf{$^{57}$Ni}} & \multicolumn{1}{c}{\textbf{$^{58}$Ni}} & \multicolumn{1}{c|}{\textbf{$^{44}$Ti}}\\ 
 \hline 
\endhead
\hline
%\multicolumn{8}{|r|}{{Continued on next page}} \\ \hline
\endfoot

\hline
\endlastfoot 

 \tableline

s10.8  &  2.71E-02  &  5.25E-04  &  1.82E-04  & 1.45E-05\\
s11.0  &  2.38E-02  &  3.46E-04  &  1.25E-04  &  1.15E-05\\
s11.2  &  2.31E-02  &  3.12E-04  &  1.01E-04  &  1.28E-05\\
s11.4  &  2.24E-02  &  3.13E-04  &  1.08E-04  &  1.08E-05\\
s11.6  &  2.43E-02  &  3.34E-04  &  1.14E-04  &  1.08E-05\\
s11.8  &  2.39E-02  &  3.70E-04  &  1.27E-04  &  1.36E-05\\
s12.0  &  3.69E-02  &  1.51E-03  &  3.58E-03  &  2.06E-05\\
s12.2  &  3.38E-02  &  7.28E-04  &  3.77E-04  &  2.32E-05\\
s12.4  &  4.06E-02  &  6.86E-04  &  2.46E-04  &  2.33E-05\\
s12.6  &  4.76E-02  &  7.00E-04  &  3.56E-04  &  2.20E-05\\
s12.8  &  3.20E-02  &  4.35E-04  &  1.54E-04  &  1.36E-05\\
s13.0  &  4.38E-02  &  1.74E-03  &  4.14E-03  &  2.07E-05\\
s13.2  &  4.83E-02  &  8.89E-04  &  2.91E-04  &  2.89E-05\\
s13.4  &  5.19E-02  &  9.72E-04  &  3.16E-04  &  3.04E-05\\
s13.6  &  5.92E-02  &  1.12E-03  &  3.82E-04  &  3.39E-05\\
s13.8  &  6.08E-02  &  1.16E-03  &  4.03E-04  &  3.54E-05\\
s14.0  &  6.85E-02  &  1.30E-03  &  4.63E-04  &  3.83E-05\\
s14.2  &  7.51E-02  &  1.46E-03  &  5.45E-04  &  4.19E-05\\
s14.4  &  8.09E-02  &  1.57E-03  &  6.17E-04  &  4.40E-05\\
s14.6  &  8.18E-02  &  1.60E-03  &  6.39E-04  &  4.53E-05\\
s14.8  &  8.66E-02  &  1.75E-03  &  7.91E-04  &  4.92E-05\\
s15.0  &  9.22E-02  &  1.79E-03  &  7.41E-04  &  4.97E-05\\
s15.2  &  1.09E-01  &  2.94E-03  &  4.48E-03  &  5.20E-05\\
s15.4  &  1.23E-01  &  2.50E-03  &  1.60E-03  &  5.70E-05\\
s15.6  &  1.08E-01  &  4.40E-03  &  1.15E-02  &  4.25E-05\\
s15.8  &  9.86E-02  &  1.72E-03  &  5.40E-04  &  4.32E-05\\
s16.0  &  7.54E-02  &  2.97E-03  &  7.41E-03  &  3.26E-05\\
s16.2  &  8.63E-02  &  3.22E-03  &  7.85E-03  &  4.02E-05\\
s16.4  &  6.90E-02  &  2.69E-03  &  6.70E-03  &  3.12E-05\\
s16.6  &  8.12E-02  &  1.23E-03  &  3.29E-04  &  3.87E-05\\
s16.8  &  7.87E-02  &  1.19E-03  &  3.28E-04  &  3.70E-05\\
s17.0  &  7.93E-02  &  1.19E-03  &  3.28E-04  &  3.77E-05\\
s17.2  &  7.95E-02  &  1.21E-03  &  3.29E-04  &  3.75E-05\\
s17.4  &  6.45E-02  &  2.52E-03  &  6.31E-03  &  3.22E-05\\
s17.6  &  7.61E-02  &  1.14E-03  &  3.30E-04  &  3.48E-05\\
s17.8  &  1.23E-01  &  5.01E-03  &  1.32E-02  &  5.30E-05\\
s18.0  &  1.12E-01  &  4.50E-03  &  1.19E-02  &  4.35E-05\\
s18.2  &  7.98E-02  &  3.13E-03  &  7.89E-03  &  3.36E-05\\
s18.4  &  9.72E-02  &  2.47E-03  &  2.85E-03  &  6.06E-05\\
s18.6  &  6.88E-02  &  2.65E-03  &  6.54E-03  &  3.10E-05\\
s18.8  &  6.90E-02  &  2.66E-03  &  6.56E-03  &  3.05E-05\\
s19.0  &  1.12E-01  &  2.35E-03  &  1.36E-03  &  6.15E-05\\
s19.2  &  1.04E-01  &  2.20E-03  &  1.26E-03  &  6.19E-05\\
s19.4  &  1.07E-01  &  4.27E-03  &  1.10E-02  &  5.17E-05\\
s19.6  &  3.56E-02  &  5.14E-04  &  2.74E-04  &  1.85E-05\\
s19.8  &  6.90E-02  &  1.05E-03  &  4.37E-04  &  3.18E-05\\
s20.0  &  6.24E-02  &  9.35E-04  &  2.92E-04  &  2.93E-05\\
s20.2  &  3.06E-02  &  4.35E-04  &  1.56E-04  &  1.61E-05\\
s20.4  &  8.16E-02  &  1.34E-03  &  3.93E-04  &  3.78E-05\\
s20.6  &  1.17E-01  &  2.08E-03  &  4.82E-04  &  5.27E-05\\
s20.8  &  1.13E-01  &  1.98E-03  &  5.08E-04  &  5.04E-05\\
s21.0  &  1.35E-01  &  2.84E-03  &  1.85E-03  &  6.14E-05\\
s21.2  &  1.15E-01  &  2.80E-03  &  3.06E-03  &  5.99E-05\\
s21.4  &  1.11E-01  &  4.34E-03  &  1.12E-02  &  4.56E-05\\
s21.6  &  8.61E-02  &  1.31E-03  &  4.46E-04  &  3.64E-05\\
s21.8  &  1.18E-01  &  2.60E-03  &  2.11E-03  &  6.01E-05\\
s22.0  &  6.91E-02  &  2.64E-03  &  6.44E-03  &  3.09E-05\\
s22.4  &  9.08E-02  &  1.42E-03  &  4.25E-04  &  3.72E-05\\
s22.6  &  1.13E-01  &  1.94E-03  &  6.49E-04  &  4.61E-05\\
s25.8  &  8.07E-02  &  1.46E-03  &  3.68E-04  &  4.16E-05\\
s26.0  &  1.28E-01  &  2.44E-03  &  5.85E-04  &  9.34E-05\\
s26.2  &  7.81E-02  &  1.30E-03  &  3.21E-04  &  4.05E-05\\
s26.4  &  8.30E-02  &  1.34E-03  &  3.22E-04  &  4.15E-05\\
s26.6  &  7.78E-02  &  1.26E-03  &  3.23E-04  &  3.96E-05\\
s26.8  &  7.98E-02  &  1.30E-03  &  7.18E-04  &  4.06E-05\\
s27.0  &  8.43E-02  &  1.39E-03  &  3.03E-04  &  4.13E-05\\
s27.2  &  8.60E-02  &  1.40E-03  &  4.35E-04  &  4.14E-05\\
s27.4  &  8.82E-02  &  1.49E-03  &  3.05E-04  &  4.34E-05\\
s27.6  &  8.93E-02  &  1.48E-03  &  3.09E-04  &  4.30E-05\\
s27.8  &  9.01E-02  &  1.50E-03  &  3.02E-04  &  4.36E-05\\
s28.0  &  8.71E-02  &  1.38E-03  &  2.91E-04  &  4.09E-05\\
s28.2  &  1.14E-01  &  4.49E-03  &  1.19E-02  &  4.71E-05\\
s29.0  &  9.81E-02  &  2.89E-03  &  5.25E-03  &  4.05E-05\\
s30.0  &  1.33E-01  &  5.45E-03  &  1.45E-02  &  5.17E-05\\
s31.0  &  8.24E-02  &  1.24E-03  &  3.54E-04  &  3.57E-05\\
s32.0  &  1.00E-01  &  1.58E-03  &  4.44E-04  &  3.83E-05\\
s33.0  &  1.07E-01  &  1.72E-03  &  4.61E-04  &  4.22E-05\\
s34.0  &  1.15E-01  &  1.95E-03  &  5.51E-04  &  4.63E-05\\
s35.0  &  9.67E-02  &  1.54E-03  &  4.14E-04  &  3.98E-05\\
s36.0  &  1.04E-01  &  1.72E-03  &  4.43E-04  &  4.07E-05\\
s37.0  &  1.58E-01  &  3.61E-03  &  3.36E-03  &  8.10E-05\\
s38.0  &  8.97E-02  &  1.44E-03  &  2.93E-04  &  4.21E-05\\
s40.0  &  8.79E-02  &  1.61E-03  &  3.71E-04  &  4.69E-05\\
s75.0  &  2.65E-02  &  4.04E-04  &  1.47E-04  &  1.50E-05\\
%\hline
 & & & & \\
w12.0   & 3.87E-02  & 1.33E-03  & 1.38E-03 &  2.37E-05\\
w13.0   & 5.50E-02  & 1.92E-03  & 2.09E-03  & 3.48E-05\\
w14.0   & 7.15E-02 &  2.51E-03 &  2.85E-03 &    4.26E-05\\
w15.0  & 1.17E-01  & 4.28E-03 &  7.60E-03   & 5.38E-05\\
w16.0  & 6.64E-02  & 2.09E-03  & 2.88E-03   & 3.02E-05\\
w17.0  & 7.03E-02  & 2.18E-03 &  2.87E-03   & 3.09E-05\\
w18.0  & 9.40E-02  & 3.58E-03  & 6.32E-03   & 5.87E-05\\
w19.0  & 8.71E-02  & 2.69E-03  & 3.26E-03   & 3.57E-05\\
w20.0  & 1.12E-01  & 3.41E-03  & 4.24E-03   & 4.92E-05\\
w21.0  & 6.22E-02  & 2.46E-03  & 6.07E-03   & 2.98E-05\\
w22.0  & 1.14E-01  & 3.49E-03  & 4.30E-03   & 4.91E-05\\
w25.0  & 1.18E-01  & 3.51E-03  & 4.69E-03   & 7.73E-05\\
w26.0  & 7.33E-02  & 2.16E-03  & 2.30E-03    & 3.73E-05\\
w27.0  & 8.62E-02  & 2.57E-03 &  3.00E-03   & 4.26E-05\\
w28.0  & 1.53E-01 &  5.84E-03  & 1.55E-02   & 6.18E-05\\
w29.0  & 9.63E-02   & 2.90E-03  & 3.68E-03   & 4.08E-05\\
w30.0 &  1.08E-01  & 3.31E-03  & 3.68E-03   & 4.27E-05\\
w31.0  & 9.93E-02 &  2.97E-03 &  3.31E-03   & 3.92E-05\\
w32.0  & 1.13E-01  & 3.39E-03 &  3.87E-03   & 4.54E-05\\
w33.0  & 1.18E-01  & 3.55E-03 &  4.19E-03   & 4.95E-05\\
w50.0 &  1.06E-01  & 3.19E-03  & 3.52E-03   & 4.15E-05\\
w55.0 &  9.97E-02  & 2.97E-03  & 3.63E-03   & 4.27E-05\\
w60.0 &  8.32E-02  & 1.27E-03  & 4.91E-04   & 5.67E-05\\
w70.0 &  9.84E-02  & 3.03E-03  & 3.78E-03   & 3.92E-05\\
w80.0 &  8.80E-02  & 2.69E-03  & 3.41E-03   & 3.55E-05\\
w100.0 & 1.23E-01  & 4.09E-03  & 5.38E-03   & 6.14E-05\\
w120.0 & 8.09E-02 &  2.56E-03  & 2.95E-03   & 3.62E-05\\

\end{longtable*}
\end{center}
